Injecting Image Guidance into Text-Conditioned Diffusion Models at Inference

Text-to-image diffusion models like Stable Diffusion generate high-quality images from text, but lack a way to inject visual guidance (e.g. sketches, styles) at inference without retraining. Existing methods either require computationally expensive fine-tuning or rely on style transfer techniques that risk semantic misalignment with textual prompts. We introduce Visual Concept Fusion (VCF), the first method offering dual conditioning on both an image and text prompt at inference time without any concept-specific training. VCF enables visual concept injection into Stable Diffusion by aligning CLIP image features with the text embedding space. VCF consists of three components: (1) a lightweight aligner that maps image tokens to the text embedding manifold using InfoNCE and cross-attention reconstruction losses, (2) a fusion strategy that preserves both textual and visual semantics, and (3) an optional Prompt-Noise Optimization (PNO) module for test-time refinement. Our experiments demonstrate that VCF successfully transfers visual attributes including style, composition, and color palette from reference images while maintaining prompt adherence. Quantitative results show a trade-off between text alignment (CLIP score) and visual correspondence (LPIPS), with VCF outperforming baselines in reference fidelity.

==> figures/ablations/scheduled_conditioning/scheduled_conditioning.tex <==

\newcommand{\resultsconditioning}[6] {
\begin{minipage}[t]{0.15\linewidth}
  \centering
  \includegraphics[width=\linewidth]{#1}
  \scriptsize Reference image
\end{minipage}
\hspace{2mm}
\begin{minipage}[t]{0.15\linewidth}
  \centering
  \includegraphics[width=\linewidth]{#2}
  \scriptsize SDv2 (text-only)
\end{minipage}
\hspace{-1mm}
\begin{minipage}[t]{0.15\linewidth}
  \centering
  \includegraphics[width=\linewidth]{#3}
  \scriptsize Conditioning Throughout
\end{minipage}
\hspace{-1mm}
\begin{minipage}[t]{0.15\linewidth}
  \centering
  \includegraphics[width=\linewidth]{#4}
  \scriptsize Conditioning First Half
\end{minipage}
\hspace{-1mm}
\begin{minipage}[t]{0.15\linewidth}
  \centering
  \includegraphics[width=\linewidth]{#5}
  \scriptsize Conditioning Second Half
\end{minipage}
\hspace{-1mm}
\begin{minipage}[t]{0.15\linewidth}
  \centering
  \includegraphics[width=\linewidth]{#6}
  \scriptsize Conditioning Middle Portion
\end{minipage}
\vspace{2mm}
}

% -----------------------------------------------------------------
% 2. Figure occupying the full text width
% -----------------------------------------------------------------
\begin{figure}[H]   % ‘p’ makes LaTeX place it on a dedicated float page
  \centering
  % Row 1 — Van Gogh
  \resultsconditioning
                {figures/ablations/scheduled_conditioning/1_1.jpg}
                {figures/ablations/scheduled_conditioning/1_2.jpg}
                {figures/ablations/scheduled_conditioning/1_3.jpg}
                {figures/ablations/scheduled_conditioning/1_4.jpg}
                {figures/ablations/scheduled_conditioning/1_5.jpg}
                {figures/ablations/scheduled_conditioning/1_6.jpg}

  % Row 2 — Picasso
  \resultsconditioning
                {figures/ablations/scheduled_conditioning/2_1.jpg}
                {figures/ablations/scheduled_conditioning/2_2.jpg}
                {figures/ablations/scheduled_conditioning/2_3.jpg}
                {figures/ablations/scheduled_conditioning/2_4.jpg}
                {figures/ablations/scheduled_conditioning/2_5.jpg}
                {figures/ablations/scheduled_conditioning/2_6.jpg}

  % Row 3 — Cat
  \resultsconditioning
                {figures/ablations/scheduled_conditioning/3_1.jpg}
                {figures/ablations/scheduled_conditioning/3_2.jpg}
                {figures/ablations/scheduled_conditioning/3_3.jpg}
                {figures/ablations/scheduled_conditioning/3_4.jpg}
                {figures/ablations/scheduled_conditioning/3_5.jpg}
                {figures/ablations/scheduled_conditioning/3_6.jpg}

  \caption{%
    Qualitative ablation on the naive fusion type, where the blended conditioning is only applied for a fraction of the diffusion sampling process.  
    Each row shows (left → right): the reference image, baseline text-only SDv2 output, blended conditioning applied on the whole diffusion procces, on the first half only, on the second half only, and on the middle portion of the diffusion process (0.3-0.7).%
  }
  \label{fig:conditioning-ablation-fullpage}
\end{figure}

